A topological-like gravity model in a four dimensional space-time

In this work we consider a model for gravity in 4-dimensional space-time originally proposed by A. Chamseddine which may be derived by a 5-dimensional Chern-Simons theory. Its topological origin makes it an interesting candidate for an easier quantization, e.g., in loop quantization framework. The present work is dedicated to classical physical consequences and canonical analysis of the model. Cosmological solutions as well as wave-like solutions were obtained and compared with the corresponding Einstein's General Relativity with cosmological constant.

==> apendice3.tex <==
 Em $1916$, um ano após a formulação final das equações da relatividade geral, Albert Einstein mostrou que suas equações faziam predições da existência de ondas gravitacionais. Ele encontrou que no regime de linearização das suas equações e de campo gravitacional fraco as equações apresentam soluções de onda: ondulações transversais do próprio tecido do espaço que se propagam na velocidade da luz. Einstein percebeu que a amplitude dessas ondas seria extremamente pequena e de difícil detecção. 
 
Duas estrelas de nêutron orbitando ao redor uma da outra devem perder energia devido à emissão de ondas gravitacionais \cite{Damour}. Essas ondas, assim como as ondas eletromagnéticas, são portadoras de energia e momento e são previstas pela teoria da Relatividade Geral. O processo de linearização das equações de Einstein gera, no famoso calibre de De Donder, equações de onda para a geometria do espaço-tempo\cite{Gasperini}. Seria como imaginar um lago sendo o espaço-tempo e, ao soltarmos uma pedra sobre este, vemos ondas que se propagam a partir da fonte emissora. Do mesmo modo, em alguns eventos gravitacionais, como por exemplo a explosão de uma Supernova, é de se esperar pelas equações que haja ondas de geometria, ou seja, flutuações geométricas em torno de um fundo geométrico que se tem \textit{a priori}.


 No mesmo ano, um brilhante astrônomo e físico alemão, o judeu chamado Karl Schwazschild, enquanto servia na Rússsia, na primeira guerra mundial, encontrou soluções exatas para as equações de Einstein. Ele escreveu um trabalho fundamental que conseguia pela primeira vez resolver de maneira exata as equações da relatividade geral para o caso particular de simetria esférica. Sua solução deu origem a uma predição sem precedentes na ciência. O espaço-tempo se assemelhando a uma cama-elástica tendo essa plasticidade e capacidade de se curvar na presença de matéria-energia, é possível concentrar tanta matéria em uma região do espaço-tempo que a curvatura, ou seja,  campo gravitacional é tão intenso que nem mesmo a luz conseguiria escapar. Essa solução foi entendida, mais tarde, através de contribuições importantíssímas do físico indiano Subrahmanyan Chandrasekhar \cite{Ash6}, como a descrição dos chamados \textit{buracos negros}, e são objetos de muito estudo e debate até hoje. Desde então experimentos a fim de se detectar ondas gravitacionais tem sido propostos e uma das possíveis fontes para a propagação dessas ondas seria um caso onde dois buracos negros que giram em torno um do outro se fundem. Esse processo de fusão de dois buracos negros seria capaz de gerar ondas gravitacionais. Seria como pensar em duas crianças brincando sobre a cama-elástica correndo de uma lado para o outro interagindo entre si, isso provocaria perturbações no tecido da cama que se propaga. E exatamente $100$ anos depois dessas predições dantes impensáveis o observatório LIGO (\textit{Laser Interferometer Gravitational-Wave Observatory}) anunciou, em Fevereiro desse ano, a descoberta mais surpreendente de todos os tempos na ciência. Um século após as predições fundamentais de Einstein e Schwarzschild foi reportado a primeira detecção direta de ondas gravitacionais advindas de um sistema binário de buracos negros fundindo em um único. Essas observações proporcionam um acesso singular, em toda história do desenvolvimento científico, as propriedades fundamentais do espaço-tempo no regime de campo gravitacional intenso e alta velocidade, e confirmando as predições da relatividade geral \cite{ligo1,ligo2}. 
 
 Devemos ter em mente que essa descoberta fantástica irá abrir uma nova janela astronômica para escrutarmos o universo que ainda não tivemos acesso\cite{louis}. Regiões que são opacas a luz ou a ondas eletromagnéticas não o são as ondas gravitacionais, daí será possível ter acesso a um conhecimento sem precedentes na ciência. As chaves do castelo cósmico foram encontradas e a nova era da cosmologia e da astronomia está por vir. Acredito que muitos mistérios poderão ser solucionados com esse novo óculos que as ondas gravitacionais nos fornecerá, alargando os limites e as condições para a produção do conhecimento da nossa história cósmica. Ao longo dos últimos trinta anos, medições acuradas tem sido realizadas a fim de testar se essas e até predições mais exóticas estão corretas. A cada vez, a Relatividade Geral tem triunfado \cite{Will,Will2}.


which are the same as achieved by our model in the linear regime. Since in the Palatini formalism for GR, without fermionic matter, one reproduces the same content as the $2^{\textrm{nd}}$-order formalism. The search for wave-like solutions in our model reduces to the analysis of perturbations around a curved background, for instance de Sitter one, in the metric formalism. Henceforth, separating the space-time metric as $g_{\mu\nu} \,=\, \mathring{g}_{\mu\nu} \,+\, h_{\mu\nu}$, with $\mid h_{\mu\nu}\mid \ll 1$ it is very straightforward to show that the first order perturbed quantities, denoting with a superscript $1$, read as
\begin{equation}
\Gamma^{\alpha (1)}\,_{\mu\nu} = \frac{1}{2}\mathring{g}^{\alpha\beta}\bigl(\mathring{\nabla}_{\mu} h_{\beta\nu} + \mathring{\nabla}_{\nu} h_{\mu\beta} - \mathring{\nabla}_{\beta} h_{\mu\nu}\bigr)
\label{eqq}
\end{equation}  
Here the raising and lowering of indices and calculation of covariant derivatives are done using the background metric $\mathring{g}_{\mu\nu}$. The expression for curvature can be obtained from Eq.(\ref{eqq}), in first order, by noting that terms like $\Gamma^{2}$ are negligible in the computation to the required order.
\begin{eqnarray}
R^{\alpha (1)}\,_{\kappa\mu\nu} & = & \frac{1}{2}\bigl(\mathring{\nabla}_{\mu}\mathring{\nabla}_{\nu}h^{\alpha}_{\kappa} + \mathring{\nabla}_{\mu}\mathring{\nabla}_{\kappa}h^{\alpha}_{\nu} - \mathring{\nabla}_{\mu}\mathring{\nabla}^{\alpha}h_{\kappa\nu} -\mathring{\nabla}_{\nu}\mathring{\nabla}_{\mu}h^{\alpha}_{\kappa} \nonumber \\ [0.1cm]
& & - \mathring{\nabla}_{\nu}\mathring{\nabla}_{\kappa}h^{\alpha}_{\mu} + \mathring{\nabla}_{\nu}\mathring{\nabla}^{\alpha}h_{\kappa\mu} \bigr)
\label{eqr}
\end{eqnarray}
Contracting the curvature tensor, we obtain the Ricci tensor, $R^{(1)}_{\alpha\kappa} \,=\, R^{\mu (1)}\,_{\alpha \mu \kappa}$,
\begin{equation}
R^{(1)}_{\alpha\kappa} = \frac{1}{2}\bigl(\mathring{\nabla}_{\mu}\mathring{\nabla}_{\kappa}h^{\mu}_{\alpha} + \mathring{\nabla}_{\mu}\mathring{\nabla}_{\alpha}h^{\mu}_{\kappa} - \mathring{\nabla}_{\mu}\mathring{\nabla}^{\mu}h_{\alpha\kappa} - \mathring{\nabla}_{\kappa}\mathring{\nabla}_{\alpha}h^{\mu}_{\mu}\bigr),
\end{equation}
since our region of interest is away from the sources $T_{\mu\nu}\,=\, 0$, \textit{i.e.}, we are considering the dynamics of the perturbations in a matter-free region. Therefore, the equation $R_{\alpha\kappa} \,=\, 0$ should be hold order by order. Demanding, $\mathring{R}_{\alpha\kappa} \,=\, 0$, we have that the background metric must be a solution of Einstein's equations in the matter-free region. The next order, $R^{(1)}_{\alpha\kappa}\,=\, 0$ gives the equations of motion obeyed by the perturbations
\begin{equation}
\mathring{\nabla}_{\mu}\mathring{\nabla}_{\kappa}h^{\mu}_{\alpha} + \mathring{\nabla}_{\mu}\mathring{\nabla}_{\alpha}h^{\mu}_{\kappa} - \mathring{\nabla}_{\mu}\mathring{\nabla}^{\mu}h_{\alpha\kappa} - \mathring{\nabla}_{\kappa}\mathring{\nabla}_{\alpha}h^{\mu}_{\mu} = 0,
\label{eqs}
\end{equation}

We now want to rewrite Eq.(\ref{eqr}) in a wave-like equation form in the curved background. We denote the trace $h^{\mu}_{\mu}$ only by $h$, and the trace-reversed metric $\bar{h}_{\mu\nu} \,=\, h_{\mu\nu} \,-\, 1/2 \mathring{g}_{\mu\nu}h$. Under a infinitesimal diffeomorphism transformation, $x^{\mu} \, \longrightarrow \, x^{\mu} \,+\, \xi^{\mu}$, the metric perturbations change as
\begin{equation}
h_{\mu\nu} \longrightarrow h_{\mu\nu} + \mathring{\nabla}_{\mu}\xi_{\nu} + \mathring{\nabla}_{\nu}\xi_{\mu},
\label{eqt}
\end{equation}
using this gauge freedom we can always impose (accessibility) conditions under the divergences of the trace-reversed metric perturbations
\begin{equation}
\mathring{\nabla}_{\mu}(h^{\mu}_{\nu} -\frac{1}{2}\delta^{\mu}_{\nu}h) = \mathring{\nabla}_{\mu}\bar{h}^{\mu\nu} = 0.
\end{equation}

Recall that
\begin{equation}
[\mathring{\nabla}_{\mu},\mathring{\nabla}_{\nu}]T^{\alpha}\,_{\beta} = \mathring{R}^{\alpha}\,_{\mu\nu\lambda}T^{\lambda}\,_{\beta} + \mathring{R}^{\lambda}\,_{\mu\nu\beta}T^{\alpha}\,_{\lambda},
\label{equ}
\end{equation}
once these conditions are imposed, we can manipulate Eq. (\ref{eqs}) making use of the relation given by Eq.(\ref{equ}) and finally 
\begin{equation}
\mathring{\square}\bar{h}_{\mu\nu} + 2\mathring{R}_{\alpha\mu\beta\nu}\bar{h}^{\alpha\beta} = 0
\label{eqq}
\end{equation}
where $\mathring{\square} \equiv \mathring{\nabla}_{\alpha}\mathring{\nabla}^{\alpha}$, is the covariant D'Alembert operator. The Eq.(\ref{eqq}) describes the propagation of a weak gravitational waves in the source-free region of a curved background spacetime. In the special case of a de Sitter background $\mathring{R}_{\mu\alpha\beta\nu}\,=\,\dfrac{\Lambda}{3}(\mathring{g}_{\mu\beta}\mathring{g}_{\alpha\nu} - \mathring{g}_{\mu\nu}\mathring{g}_{\alpha\beta})$, the wave equation reads\footnote{Recall that the trace-reversed metric $\bar{h}_{\mu\nu}$ has the inverse of the trace of $h_{\mu\nu}$. To see this, since $\bar{h}_{\mu\nu} = h_{\mu\nu} -1/2 \mathring{g}_{\mu\nu}h$ $\longmapsto$ $\bar{h} = \mathring{g}^{\mu\nu}\bar{h}_{\mu\nu} = -h$.} 
\begin{equation}
\mathring{\square}\bar{h}_{\mu\nu} + \frac{2\Lambda}{3}(\bar{h}_{\mu\nu} + \mathring{g}_{\mu\nu}h) = 0.
\end{equation}
